ZET-Speech: Zero-shot adaptive Emotion-controllable Text-to-Speech Synthesis with Diffusion and Style-based Models

Emotional Text-To-Speech (TTS) is an important task in the development of systems (e.g., human-like dialogue agents) that require natural and emotional speech. Existing approaches, however, only aim to produce emotional TTS for seen speakers during training, without consideration of the generalization to unseen speakers. In this paper, we propose ZET-Speech, a zero-shot adaptive emotion-controllable TTS model that allows users to synthesize any speaker's emotional speech using only a short, neutral speech segment and the target emotion label. Specifically, to enable a zero-shot adaptive TTS model to synthesize emotional speech, we propose domain adversarial learning and guidance methods on the diffusion model. Experimental results demonstrate that ZET-Speech successfully synthesizes natural and emotional speech with the desired emotion for both seen and unseen speakers. Samples are at https://ZET-Speech.github.io/ZET-Speech-Demo/.

==> texts/2_related_work.tex <==
\section{Related Works}
Generating emotional speech has been a topic of considerable interest in TTS research, with numerous studies investigating various methods to achieve this goal.
In this section, we discuss several noteworthy works in emotional TTS and elucidate the unique aspects of our approach in comparison to these works.

The most active research area is \textbf{cross-speaker emotion (style) transfer} where the goal is to transfer the emotion of the source speaker to the target speaker.
Global Style Token~\cite{StyleToken} is one of the famous works in this field and various follow-up studies develop the method with prosody bottleneck~\cite{cs1}, condition layer normalization~\cite{cs2}, prosody features from pre-trained speech recognition model~\cite{cs3}, and data augmentation with voice conversion model~\cite{cs4}. 
Beyond referenced works, there are a lot of existing works that tackle the cross-speaker emotion transfer problem.
The key to this task is to remove the speaker identity from the source speech and only transfer the prosody feature to the target speaker's synthesized speech.
Therefore, the aforementioned works are orthogonal to ours since they neither tackle the zero-shot scenario where the target speakers are not trained nor consider the case only with emotion labels.
There are few works~\cite{styletag, styletag2} consider the case only with emotion labels in natural language (style tag), but they also focus only on single or cross-speaker settings where the TTS model cannot be applied to unseen speakers.

Another direction is the \textbf{intensity controllable} emotional TTS.
Previous works~\cite{eic1,eic2} propose to mix the style embeddings to control the emotional intensity of the synthesized speech.
Recently, EmoDiff~\cite{EmoDiff} propose to utilize the classifier guidance to synthesize intensity controllable emotional speech only with a single speaker.
Apparently, those works are also highly orthogonal to our work since we do not focus on intensity control. 



